Content-Based Weak Supervision for Ad-Hoc Re-Ranking

One challenge with neural ranking is the need for a large amount of manually-labeled relevance judgments for training. In contrast with prior work, we examine the use of weak supervision sources for training that yield pseudo query-document pairs that already exhibit relevance (e.g., newswire headline-content pairs and encyclopedic heading-paragraph pairs). We also propose filtering techniques to eliminate training samples that are too far out of domain using two techniques: a heuristic-based approach and novel supervised filter that re-purposes a neural ranker. Using several leading neural ranking architectures and multiple weak supervision datasets, we show that these sources of training pairs are effective on their own (outperforming prior weak supervision techniques), and that filtering can further improve performance.

==> tab_aol.tex <==
\begin{table}
\small
\caption{Comparison of training approaches on the ranking-based source (AOL) on WT12. Our approach is \textit{cutoff}, and we compare to the \textit{scores} and \textit{pairs} approaches proposed by~\cite{dehghani2017neural}. The top result for each model is listed in bold. Significant performance reductions compared to the cutoff approach are marked with $\downarrow$ (paired t-test, $p<0.05$).}
\label{tab:ranking-based-approaches}
\begin{tabular}{llll}
\toprule
Model & \multicolumn{3}{c}{nDCG@20}\\ \cmidrule(lr){2-4} 
        &cutoff & scores~\cite{dehghani2017neural} & pairs~\cite{dehghani2017neural} \\
\midrule


Conv-KNRM & 0.1498 & 0.1533 & \bf0.1567  \\
PACRR & \bf0.1910 & 0.1192 $\downarrow$ & 0.1704  \\
MatchPyramid & \bf0.1327 & 0.1026 & 0.1249  \\
KNRM & \bf0.1782 & 0.0969 $\downarrow$ & 0.1705  \\
DRMM & 0.1380 & \bf0.1614 & 0.1574  \\
DUETL & \bf0.0991 & 0.0705 $\downarrow$ & 0.0512 $\downarrow$ \\


\bottomrule
\end{tabular}
\end{table}

==> tab_final.tex <==
\begin{table}
\centering
\small
\caption{Caption}
\begin{tabular}{lrrrr}
\toprule
&\multicolumn{4}{c}{WebTrack 2012-14, nDCG@20} \\\cmidrule(lr){2-5}
        Model & \cellcolor{black!15} BM25 & WT10 & WT (all) & Ours (best) \\
\midrule



PACRR & \cellcolor{black!15} & 0.2272 & 0.2754 & \bf 0.2875 \\
Conv-KNRM & 0.1970  \cellcolor{black!15} & 0.2392 & \bf 0.2899 & 0.2697 \\
KNRM & \cellcolor{black!15} & 0.2658 & \bf 0.2707 & 0.2389 \\


\bottomrule
\end{tabular}
\label{tab:my_label}
\end{table}


==> tab_finetune.tex <==
\begin{table}
\centering
\caption{WT14 results for fine-tuning performance on the NYT dataset using WT10 data for a final stage of training. The top score for each model are listed in bold.% Significant reductions compared to training on only NYT data  are marked with $\downarrow$ (paired t-test, $p<0.05$).
}
\label{tab:finetune}
\begin{tabular}{lrr}
\toprule
Model & \multicolumn{2}{c}{nDCG@20}\\ \cmidrule(lr){2-3} 
        &NYT & NYT+WT10 \\
\midrule



Conv-KNRM & 0.3215 & \bf0.3216 \\
PACRR & 0.3016 & \bf0.3050 \\
MatchPyramid & 0.2825 & \bf0.2934 \\
KNRM & \bf0.2865 & 0.2828 \\
DRMM & 0.1963 & \bf0.2115 \\
DUETL & \bf0.2550 & 0.1912 \\



\bottomrule
    \end{tabular}
\end{table}


==> tab_nyt_content.tex <==
\begin{table}
\centering
\small
\caption{Comparison between the ranking performance when NYT is used as a content-based source (NYT-content) verses when it is used as a ranking-based source (NYT-ranking, as done by~\cite{Li2018JointLF}). The top score for each model within each evaluation dataset is listed in bold. Significant reductions in performance for NYT-content are marked with $\downarrow$ (paired t-test, $p<0.05$).}
\label{tab:results-nyt-as-content}
\begin{tabular}{lllll}
\toprule
Model &   Training & \multicolumn{3}{c}{nDCG@20}\\ \cmidrule(lr){3-5} 
        &&WT12 & WT13 & WT14 \\
\midrule


Conv-KNRM & NYT-content & \bf0.2637  & 0.2031 \\
 & NYT-ranking & 0.2473 $\downarrow$ & \bf0.2085 \\
\midrule
PACRR & NYT-content & \bf0.2690  & \bf0.2136 \\
 & NYT-ranking & 0.2622  & 0.2029 \\
\midrule
KNRM & NYT-content & 0.2220  & 0.1536 \\
 & NYT-ranking & \bf0.2244  & \bf0.1792 $\uparrow$\\
\midrule
DRMM & NYT-content & 0.1375  & 0.1000 \\
 & NYT-ranking & \bf0.1484  & \bf0.1078 \\


\bottomrule
    \end{tabular}
\end{table}

==> tab_validation.tex <==
\begin{table}
\centering
\small
\caption{Performance results when using a held-out set of NYT data as validation instead of in-domain WT11 data. The top score for each model within each evaluation dataset is listed in bold. Significant reductions in performance for NYT-content are marked with $\downarrow$ (paired t-test, $p<0.05$).}
\label{tab:validation}
\begin{tabular}{lllll}
\toprule
Model &   Validation & \multicolumn{3}{c}{nDCG@20}\\ \cmidrule(lr){3-5} 
        &&WT12 & WT13 & WT14 \\
\midrule



Conv-KNRM & WT11 & \bf0.2637  & \bf0.2031 \\
 & NYT held out & 0.2390 $\downarrow$ & 0.1706 $\downarrow$\\
\midrule
PACRR & WT11 & \bf0.2690  & \bf0.2136 \\
 & NYT held out & 0.2661  & 0.2082 \\
\midrule
KNRM & WT11 & \bf0.2220  & \bf0.1536 \\
 & NYT held out & 0.2182  & 0.1530 \\
\midrule
DRMM & WT11 & 0.1375  & 0.1000 \\
 & NYT held out & \bf0.1502  & \bf0.1090 \\
 
 
 

\bottomrule
    \end{tabular}
\end{table}
